Rethinking Clause Management for CDCL SAT Solvers

Boolean Satisfiability (SAT) solving underpins a wide range of applications in Electronic Design Automation (EDA), particularly formal verification. However, this paper observes that the mainstream clause reduction heuristic in modern SAT solvers becomes ineffective in the critical domain of complex arithmetic circuit verification, such as multipliers. On these instances, the dominant Literal Block Distance (LBD) metric for measuring clause quality degrades into a simple value of clause length, without any perception of dynamic clause usage during solving. To address this issue, a novel clause reduction mechanism is proposed, which is entirely independent of LBD. Its core idea is to decouple and handle separately the two most fundamental characteristics of learnt clauses--inherent lineage and dynamic usage patterns--thereby avoiding the efficiency degradation caused by inappropriately mixing these properties. Experiments show that our method consistently improves mainstream solvers and achieves speedups of up to 5.74x on complex arithmetic circuit problems, while maintaining comparable performance on general-purpose benchmarks. These results challenge the prevailing LBD-centric clause quality metric for clause management.

==> 01_introduction.tex <==
\section{Introduction} \label{Sec:Intro}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/NotMult.png}
        \caption{General Equivalence Checking Instance}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/Mult.png}
        \caption{Multiplier Equivalence Checking Instance}
        \label{fig:sub2}
    \end{subfigure}
    \caption{Learnt Clause Distribution Analysis: LBD vs. Length in General and Multiplier Equivalence Checking}
    \label{fig:motivation}
    \vspace{-10pt}
\end{figure*}

% Multiplier equivalence checking is of significant importance to both the EDA industry and the SAT research community. As multipliers are widely deployed in performance-critical datapaths and aggressively optimized to meet stringent power, performance, and area (PPA) targets, their equivalence verification becomes both crucial and computationally challenging. In recent years, the SAT sweeping framework has emerged as a widely adopted approach to equivalence checking, owing to its ability to provide efficient solutions to such instances~\cite{mishchenko2006improvements,chen2023cnf}. However, its solving performance is highly dependent on the underlying SAT solvers employed. Consequently, the performance of SAT solvers in multiplier equivalence checking warrants careful attention. The equivalence checking of multipliers exhibits the characteristic of small scale yet high computational difficulty, thus rendering the efficient resolution of such instances of paramount academic significance within the SAT community. It is quite conceivable that a hypothetical breakthrough in CDCL performance on multiplier benchmarks would likely be regarded as another landmark achievement in the advancement of solver technology~\cite{kondratiev2024benchmarks}.

% Formal verification is of significant importance in the EDA domain, with logical equivalence checking (LEC) of circuits being particularly critical. In recent years, the SAT sweeping framework has been widely adopted owing to its ability to provide efficient solutions to such instances~\cite{mishchenko2006improvements,chen2023cnf}. However, within the SAT sweeping process, datapath circuit verification poses substantial challenges, with the primary difficulty centering on verifying incomplete multiplier subcircuits across pre- and post-synthesis stages. Since the performance of SAT sweeping tools is highly dependent on the underlying SAT solvers employed, the performance of SAT solvers in multiplier equivalence checking warrants careful attention. The equivalence checking of multipliers exhibits the characteristic of small scale yet high computational difficulty, thus rendering the efficient resolution of such instances of paramount academic significance within the SAT community. Consequently, a hypothetical breakthrough in CDCL performance on multiplier benchmarks would likely be regarded as another landmark achievement in the advancement of solver technology~\cite{kondratiev2024benchmarks}.

% Formal verification is of significant importance in the EDA domain, with logical equivalence checking (LEC) of circuits being particularly critical. In recent years, the SAT sweeping framework has been widely adopted owing to its ability to provide efficient solutions to such instances~\cite{mishchenko2006improvements,chen2023cnf}. However, within the SAT sweeping process, datapath circuit verification poses substantial challenges, with the primary difficulty centering on verifying incomplete complex arithmetic subcircuits(Represented by multiplier and divider circuits) across pre- and post-synthesis stages. Since the performance of SAT sweeping tools is highly dependent on the underlying SAT solvers employed, the performance of SAT solvers in  arithmetic circuit equivalence checking warrants careful attention. The equivalence checking of arithmetic circuits, typically multipliers, exhibits the characteristic of small scale yet high computational difficulty, thus rendering the efficient resolution of such instances of paramount academic significance within the SAT community. Consequently, a hypothetical breakthrough in CDCL performance on this kind of benchmarks would likely be regarded as another landmark achievement in the advancement of solver technology~\cite{kondratiev2024benchmarks}.

Formal verification is of significant importance in the EDA domain, with logical equivalence checking (LEC) of circuits being particularly critical. In recent years, the SAT sweeping framework has been widely adopted owing to its ability to provide efficient solutions to such instances~\cite{mishchenko2006improvements,chen2023cnf}. However, within the SAT sweeping process, datapath circuit verification poses substantial challenges, with the primary difficulty centering on verifying incomplete complex arithmetic subcircuits, represented by multiplier and divider circuits, across pre- and post-synthesis stages. Since the performance of SAT sweeping tools is highly dependent on the underlying SAT solvers employed, the performance of SAT solvers in complex arithmetic circuit equivalence checking warrants careful attention. The equivalence checking of complex arithmetic circuits, particularly multipliers, exhibits the characteristic of small scale yet high computational difficulty, thus rendering the efficient resolution of such instances of paramount academic significance within the SAT community. Consequently, a hypothetical breakthrough in CDCL performance on such benchmarks would likely be regarded as another landmark achievement in the advancement of solver technology~\cite{kondratiev2024benchmarks}.
 
 % Datapath circuit verification presents substantial challenges, with the primary difficulty lying in verifying incomplete multiplier subcircuits across pre- and post-synthesis stages.


% Mainstream SAT solvers, such as Kissat, CaDiCaL, and MiniSAT~\cite{biere2024cadical, sorensson2005minisat}, employ heuristics optimized for general-purpose instances. However, the structural properties of multiplier verification problems differ markedly from typical SAT benchmarks, rendering these heuristics less effective. In this work, we focus on the clause reduction mechanism employed by state-of-the-art (SOTA) solvers, exemplified by Kissat, which typically uses LBD (Literal Block Distance)~\cite{audemard2009glucose} as the primary criterion for clause retention decisions. LBD has been regarded as the preeminent clause quality metric for general-purpose problems for over 15 years, largely attributed to its ability to organically integrate a clause's inherent lineage (size) with its dynamic usage patterns (decision propagation), thereby providing comprehensive quality assessment. However, in this work, we observe that in the specific domain of multiplier equivalence checking, LBD's ability to integrate these two aspects has significantly deteriorated and is no longer organic. Fig.~\ref{fig:motivation} presents the distributions of learned clauses with respect to LBD and length for Kissat solver on a non-multiplier equivalence checking instance and a multiplier equivalence checking instance, respectively. It can be observed that the latter exhibits an extremely high proportion of learned clauses with LBD equal to length minus 1 (note that according to the definition of LBD, for non-unit clauses, the LBD value must be less than or equal to length minus 1), while the former shows no such trend. This demonstrates that multiplier problems exhibit fundamentally different characteristics compared to general equivalence checking problems, and LBD can no longer organically integrate a clause's inherent lineage with its dynamic usage patterns. Therefore, continuing to use LBD as the primary evaluation criterion is no longer appropriate.

% Mainstream SAT solvers, such as Kissat, CaDiCaL, and MiniSAT~\cite{biere2024cadical, sorensson2005minisat}, are designed for general-purpose instances. The effectiveness of their core pillar algorithm, CDCL, largely stems from its ability to learn clauses during conflicts for pruning, so clause management is a key factor ensuring the efficiency of CDCL. The clause reduction mechanism employed by state-of-the-art (SOTA) solvers typically use LBD (Literal Block Distance, defined as the number of distinct decision levels of the variables in the clause.)~\cite{audemard2009glucose} as the primary criterion for clause retention decisions. LBD is a heuristic that incorporates decision-level information during the solving process, and its value is naturally correlated with the number of variables in a clause. As such, LBD organically integrates a clause's inherent lineage (size) with its dynamic usage patterns (decision propagation), providing comprehensive quality assessment. This integration is the core reason why LBD has been regarded as the preeminent clause quality metric for general-purpose problems for over 15 years. However, since the structural properties of complex arithmetic circuits differ markedly from typical SAT benchmarks, we observe that in this specific domain, LBD's ability to integrate these two aspects has significantly deteriorated and is no longer organic. Fig.~\ref{fig:motivation} presents the distributions of learned clauses with respect to LBD and length for Kissat solver on a general equivalence checking instance and a multiplier equivalence checking instance, respectively. It can be observed that the latter exhibits an extremely high proportion of learned clauses with LBD consistent with its length\footnote{As learned clause generation requires at least one propagation, non-unit learned clauses have LBD $\leq$ length $-$ 1. We define LBD being consistent with length as when LBD equals length minus 1.}, while the former shows no such trend. This demonstrates that complex arithmetic problems exhibit fundamentally different characteristics compared to general equivalence checking problems, and LBD can no longer organically integrate a clause's inherent lineage with its dynamic usage patterns. Therefore, continuing to use LBD as the primary evaluation criterion is no longer appropriate.

Mainstream SAT solvers, such as Kissat, CaDiCaL, and MiniSAT~\cite{biere2024cadical, sorensson2005minisat}, are designed for general-purpose instances. The effectiveness of their core CDCL algorithm largely stems from learning clauses during conflicts for pruning, making clause management crucial for efficiency. State-of-the-art (SOTA) solvers employ LBD (Literal Block Distance, the number of distinct decision levels in a clause)~\cite{audemard2009glucose} as the primary criterion for clause retention. LBD is a heuristic that incorporates decision-level information and is naturally correlated with clause length, thus organically integrating a clause's inherent lineage (length) with its dynamic usage patterns (decision propagation). This integration explains why LBD has been the preeminent clause quality metric for general-purpose problems for over 15 years. However, since the structural properties of complex arithmetic circuits differ markedly from typical SAT benchmarks, we observe that in this domain, LBD's ability to integrate these two aspects has significantly deteriorated. Fig.~\ref{fig:motivation} presents the distributions of learned clauses with respect to LBD and length for Kissat on a general equivalence checking instance and a multiplier equivalence checking instance, respectively. The latter exhibits an extremely high proportion of learned clauses with LBD consistent with its length\footnote{Since learned clause generation involves at least one propagation, non-unit learned clauses have LBD $\leq$ length $-$ 1. We define LBD as consistent with length when LBD = length $-$ 1.}, while the former shows no such trend. This demonstrates that complex arithmetic problems exhibit fundamentally different characteristics compared to general equivalence checking problems, and LBD can no longer organically integrate a clause's inherent lineage with its dynamic usage patterns. Therefore, continuing to use LBD as the primary evaluation criterion is no longer appropriate.

 
Based on the above observations, in this work, we propose a novel two-stage clause reduction algorithm. The core idea lies in completely decoupling and separately handling the two most fundamental characteristics of learned clauses—inherent lineage and dynamic usage patterns—thereby avoiding the efficiency degradation caused by the inappropriate mixing of these two essential properties. In the first stage, we focus exclusively on the actual usage patterns of learned clauses, maximizing the retention of clauses that have demonstrated superior performance through the only two mechanisms by which clauses can influence solver behavior: Boolean Constraint Propagation (BCP) and conflict analysis. For clauses that have not yet demonstrated their potential, we rely solely on clause lineage (i.e., clause length) in stage 2 to break ties, giving promising but underutilized clauses an opportunity to prove themselves and minimizing the risk of erroneous deletion. Specifically, the main contributions of our work include:

\begin{itemize}
    \item  We challenge the supremacy of LBD, the dominant clause quality metric that has held sway for over fifteen years, particularly in the domain of multiplier verification problems.
    \item We propose completely decoupling clause lineage from actual usage patterns, and design a novel clause reduction mechanism that is entirely independent of LBD.
    \item We validate the effectiveness of our method on complex datapath arithmetic units, represented by multipliers, through detailed experiments, and conduct comprehensive data analysis.
\end{itemize}
We integrate our algorithm into mainstream SAT solvers and validate its effectiveness on both complex arithmetic verification and general-purpose benchmarks. Experimental results demonstrate that our method consistently improves solver performance on complex arithmetic verification problems, reducing Kissat's PAR2 score by approximately 40\,\% and nearly doubling the number of instances successfully solved by MiniSAT. On instances that neither timeout before nor after integrating our method, our approach achieves up to 5.74× speedup and an average speedup of 3.88× on MiniSAT. Furthermore, on the 2022 SAT Competition benchmarks, our method enables Kissat to solve 4 additional instances with a 4.7\,\% PAR2 score reduction, demonstrating significant improvement on arithmetic verification problems without compromising performance on other domains.


